Constrained Dominant sets and Its applications in computer vision

In this thesis, we present new schemes which leverage a constrained clustering method to solve several computer vision tasks ranging from image retrieval, image segmentation and co-segmentation, to person re-identification. In the last decades clustering methods have played a vital role in computer vision applications; herein, we focus on the extension, reformulation, and integration of a well-known graph and game theoretic clustering method known as Dominant Sets. Thus, we have demonstrated the validity of the proposed methods with extensive experiments which are conducted on several benchmark datasets.

==> chapters/summary.tex <==
\chapter*{Preface}
%\lettrine{S}{ummary} goes here.
\lettrine{T}his dissertation presents applications of a graph theoretic clustering framework, namely dominant sets and its variants, in solving problems in computer vision and pattern recognition. Chapter 3 presents the first application of dominant sets to solve tracking problem in a single camera. This led to the first publication \cite{YonEyaPelPraIET2016}. Chapter 4 introduces a new multi-target tracking approach in a multiple non-overlapping camera using constrained dominant sets. This work is under review at Transactions on Pattern Analysis and Machine Intelligence (TPAMI) [the arXiv version is in \cite{YonieyaPAMICDSC_tracker}] and has been developed in the last year of my PhD course, during my second visit to the Center for Research in Computer Vision (CRCV) at University of Central Florida, under the supervision of Dr. Mubarak Shah. Chapter 5 presents a Nobel approach to solve another yet very challenging computer vision problem, i.e., large scale image geo-localization using (constrained) dominant set clustering framework. The result has been published in TPAMI \cite{eyasuPAMIgeoloc}. This work is done during my first visit to CRCV at UCF. Finally, the last chapter of the thesis is devoted to outlier detections, we used some properties of dominant sets to simultaneously solve clustering and outlier detections from data. This work has been presented in \cite{zemene2016simultaneous}.


